Utilizing Remote Sensing to Analyze Land Usage and Rice Planting Patterns

The cooperative management of rice terraces in Bali reveals an interesting phenomenon that stems from the feedback loop between human decisions and the ecosystem process. In particular, spatial patterning is observed, which is heavily reliant on the farmer's decision to plant crops as well as the response from the physical environment like pest damage and water shortage. A recent study proposed an evolutionary game theoretic model to infer particular power laws governing this spatial patterning along the Bali region. In this paper, we show a snapshot of rice patches in Bali with colors to indicate the different stages of rice growth

==> abstract.tex <==
\begin{abstract}
%While vehicular sensor networks (VSNs) have \mt{earned the stature} of a mobile sensing \mt{paradigm} utilizing sensors built into cars, they have limited sensing scopes since car drivers only opportunistically discover new events. Conversely, social sensing is emerging as a new sensing paradigm where measurements about the physical world are collected from humans. In contrast to VSNs, social sensing is more pervasive, but one of its key limitations lies in \mt{its inconsistent reliability stemming from the} data contributed by unreliable human sensors. In this paper, we introduce DASC, a road damage-aware social-media-driven car sensing framework that exploits the collective power of social sensing and VSNs for reliable disaster response applications. However, integrating VSNs with social sensing introduces \mt{a new} set of challenges: \mt{i) How to} leverage the noisy and unreliable social signals to route the vehicles to the accurate regions of interest? \mt{ii) How to tackle the} inconsistent availability (e.g., churns) caused by car drivers being rational actors? \mt{iii) How to efficiently guide the cars without prior knowledge of the road damage caused by the disaster, while also handling the dynamics of the physical world and social media?} \mt{The DASC framework addresses the above challenges by establishing a novel hybrid social-car sensing system that employs techniques from game theory, feedback control, and reinforcement learning. In particular, DASC distills signals emitted from the social media and spontaneously discovers the road damages to effectively drive cars to target areas for verifying the emergency events.} \rd{We implement and evaluate DASC in a reputed vehicle simulator that can emulate real-world scenarios.} The results on a real-world disaster recovery case study \mt{demonstrate the superiority of DASC over} current VSNs-based solutions \rd{in detection effectiveness and deadline hit rate}.
\end{abstract}
 
 \begin{keyword}
Remote sensing, satellite imagery, rice planting.
\end{keyword}

 
